Designing, Building, and Characterizing RF Switch-based Reconfigurable Intelligent Surfaces

In this paper, we present our experience designing, prototyping, and empirically characterizing RF Switch-based Reconfigurable Intelligent Surfaces (RIS). Our RIS design comprises arrays of patch antennas, delay lines and programmable radio-frequency (RF) switches that enable passive 3D beamforming, i.e., without active RF components. We implement this design using PCB technology and low-cost electronic components, and thoroughly validate our prototype in a controlled environment with high spatial resolution codebooks. Finally, we make available a large dataset with a complete characterization of our RIS and present the costs associated with reproducing our design.

==> lectures.tex <==
\section{lessons learned}

1
Small deviations in the input parameters of models characterizing the characteristic impedance of microstrips yield large empirical errors.


2
Conventional models differ substantially from (full-wave) simulations when estimating the optimal depth of the notch.


3
The operating frequency of patch antennas is very sensitive to deviations in the permittivity $\epsilon_r$ of the substrate material. PCB manufacturers provide a range of $\epsilon_r$ values rather than a precise value, which may lead to large performance errors. Hence, it is worth investing time during the design phase to empirically estimate an accurate $\epsilon_r$ value for the substrate of choice.


4
Precise knowledge of  $v_{\mu \text{strip}}$ is fundamental to design the length of delay lines, and TDR is an essential technique for this purpose. However, for TDR to provide accurate measurements, the samples of microstrips under test should allow the RF signal to travel a distance larger than $2\lambda$. 


5
The ports of the RF switch have a 0.2-mm width, which is smaller than the width of the microstrip lines (0.75~mm). To minimize power loss, it is vital to implement a \emph{smooth} transition, as depicted in Fig.~\ref{fig:RFconnection}~\cite[Table 6]{smooth_line}.


6
The power gain achieved from beamforming scales with the number of cells~\cite{RISMA}. As a consequence, there is a trade-off between the efficiency of an antenna array (negligible mutual coupling when $d_{max} \ge \lambda/2$~\cite{balanis}) and the density of cells in a RIS (higher when $d_{max}\ll\lambda/2$). 
%
Hence, $d_{max} =\lambda/2$ is usually selected. However, mild power loss due to small coupling effects when $d_{max} \lesssim \lambda/2$ may be compensated by the extra cells that this choice permits~\cite{gradoni2021end}.


7
At the beginning of \S\ref{sec:prototype}, we suggested that thin substrates maximize performance. However, we learned that overly thin substrates are considerably harder to manage when assembling electronic components and tend to suffer physical distortions such as warping. 

8
It is conventionally agreed that far-field conditions are ideal for radio characterization. However, doing so for sub-6GHz arrays may be prohibitive. We learned that operating in near-field is good enough as long as we operate beyond the \emph{reactive} near-field threshold, which is less stringent than that of far-field. Prior work usually ignores this aspect~\cite{dai2020reconfigurable, pei2021ris}, which may lead to bad performance.
%Characterizations should be performed in far-field, but for sub-6GHz arrays this is prohibitive because it is in the range of couple of meters. In the literature it is common to carry it out in reactive near-field, but we moved out that zone to get results closer to the theory.  


Considering the size of the codebook and the quasi-static nature of the environment, we learned that collecting 30 samples at a sampling rate of $0.25$~ms$^{-1}$ is a good trade-off between speed and quality of information.  

==> related.tex <==
%\section{Related Work \ags{target: 0.5 column}}\label{sec:related}


%In this section a brief overview of the RIS prototypes present in the literature are given. In \cite{yezhen2020novel} a 16x16 RIS for 28GHz operating frequency, made of patch antennas connected to a PIN diode which allows only 1-bit resolution phase shift. The maximum scan angle is $\pm$60$^\circ$ and the gain is 21.7dBi. The technology used to control elements is FPGA which permits 2$\mu$s but it increases the overall power consumption with respect to a MCU, in fact the power needed to supply the RIS is 0.8W. \textcolor{blue}{Last sentence not in the paper, from my notes of Sony Lund experience, up to u to keep it.}. The authors of \cite{trichopoulos2021design} show a 16x10 RIS fabricated for 5.8 GHz and the phase shift realized with 1-bit PIN diodes. This prototype does not allow to singularly configure the elements. The control unit, an Arduino MEGA2560, does not support such an amount of elements to be set, therefore the units elements are grouped where each group of 5 elements are configured with the same phase shift. This RIS can achieve a $\pm$60$^\circ$, a bandwidth of 100 MHz and 20dB SNR in some scenarios. In \cite{tan2018enabling}, a RIS prototype consisting of 14x16 reflectors is presented with center frequency at 60 GHz. The unit elements are place more than one wavelength away to reduce the mutual coupling at the expense a tight maximum scanning angle. To set the phase shifts, a switch is involved: when it is open, the patch is isolated from the ground plane and it is reflecting, when it is closed, the antenna is shorted to the ground and it has minimum reflection. However the authors of this paper do not show any characterization of their RIS. Several MIMO prototypes are described in \cite{clerckx2022foundations} for wireless power transfer purposes and a RIS designed is shown to enhance the efficiency and extend the operational range. The adapted RIS contains 16x16 elements working at 5.8GHz equipped with a PIN diode for 1-bit control. The unit cells are controlled by a FPGA which sets the phase shift in shift registers. Unfortunately no information is given about the performance of this RIS. Of particular interest is the prototype presented in \cite{dai2020reconfigurable} because a 2-bit phase quantization is obtained using 5 PIN diodes. The RIS consists of 3 layers: the ground, the slotted plane, and the patch reflector. The length of the resonant slots is changed by activating the diodes and therefore applying different phase delay. This prototype has 16x16 elements and it is command by an FPGA. The achievable gain at 2.4 GHz is 21dBi and the main beam can be scanned up to $\pm$60$^\circ$. Also it is stated that if the radiated power is 18dB, the RIS power consumption is 153 W. In \cite{arun2020rfocus}, 40 reflectors are mounted on the boards, they are $\lambda/4$ tall, $\lambda/10$ wide and separated $\lambda/10$ on x-axis and on the y-axis just enough to connected by an RF-switch. When the switch is turned on, they reflectors form an half dipole antenna resonating at 2.4GHz. The authors put together 80 boards but they did not disclose the key parameters. A very peculiar layout was created in \cite{pei2021ris}, where a 3-layered RIS with 1100 elements is revealed that operates at 5.8GHz. An unit element consists of 4 reflectors where a PIN diode link the first two reflectors and another diode the second two. By changing the biasing voltage the authors claim the continuous phase shifts in a span of 180$^\circ$ is possible, but they limit their choice to only two value to apply a 1-bit phase shift. Given they high quantity of elements in the board, all the units on the same column are grouped together and set by an FPGA with the same phase shift. It is noteworthy the 500m field trial where a film was streamed smoothly, the RIS allowed power gain of 14 dB. The total power consumption for this RIS is 0.9W. A very similar approach is illustrated in \cite{scattermimo} to allow singular configuration of the elements reducing the number of utilized pins at controller side. This RIS is made of 4x4 patch antennas operating at 5 GHz and controlled with 2-bit phase shifter made with the transmission line method. They claim that this prototype can double the average throughput gain and increase the coverage from 30m to 45m in indoor environment. The total power consumption for it 12mW.

==> wintech/Definitions.tex <==
%=========================================================================
% Miscellaneous - Placido
%=========================================================================
%\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
%\DeclarePairedDelimiter\norm{\lVert}{\rVert}%
\newcommand{\bs}[1]{\boldsymbol{#1}}%
\newcommand{\roundP}[1]{\left(#1\right)}%
\newcommand{\squareP}[1]{\left[#1\right]}%
\newcommand{\normS}[1]{\norm{#1} ^2}%
\newcommand{\smo}[1]{\smashoperator[r]{#1}}%
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\rmm}[1]{\mathrm{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\st}{\mathrm{subject~to}}

\makeatletter
\let\oldabs\abs
\def\abs{\@ifstar{\oldabs}{\oldabs*}}

\let\oldnorm\norm
\def\norm{\@ifstar{\oldnorm}{\oldnorm*}}
\makeatother
%=========================================================================
% VECTORS
%=========================================================================
\renewcommand{\a}{\mathbf{a}}
\renewcommand{\b}{\mathbf{b}}
\renewcommand{\c}{\mathbf{c}}
\renewcommand{\d}{\mathbf{d}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\h}{\mathbf{h}}
\renewcommand{\i}{\mathbf{i}}
\renewcommand{\j}{\mathbf{j}}
\renewcommand{\k}{\mathbf{k}}
%\renewcommand{\l}{\mathbf{l}}
\newcommand{\m}{\mathbf{m}}
\newcommand{\n}{\mathbf{n}}
\renewcommand{\o}{\mathbf{o}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\q}{\mathbf{q}}
\renewcommand{\r}{\mathbf{r}}
\newcommand{\s}{\mathbf{s}}
\renewcommand{\t}{\mathbf{t}}
\renewcommand{\u}{\mathbf{u}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}

\newcommand{\0}{\mathbf{0}}
\newcommand{\1}{\mathbf{1}}


%=========================================================================
% MATRICES
%=========================================================================
\newcommand{\A}{\mathbf{A}}
\newcommand{\B}{\mathbf{B}}
%\newcommand{\C}{\mathbf{C}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\F}{\mathbf{F}}
%\newcommand{\G}{\mathbf{G}}
\renewcommand{\H}{\mathbf{H}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\K}{\mathbf{K}}
\renewcommand{\L}{\mathbf{L}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\N}{\mathbf{N}}
\renewcommand{\O}{\mathbf{O}}
\renewcommand{\P}{\mathbf{P}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\T}{\mathbf{T}}
%\newcommand{\U}{\mathbf{U}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\Z}{\mathbf{Z}}


%=========================================================================
% BOLD GREEK VARIABLES
%=========================================================================
\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\epsilonb}{\boldsymbol{\epsilon}}
\newcommand{\varepsilonb}{\boldsymbol{\varepsilon}}
\newcommand{\zetab}{\boldsymbol{\zeta}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\varthetab}{\boldsymbol{\vartheta}}
\newcommand{\iotab}{\boldsymbol{\iota}}
\newcommand{\kappab}{\boldsymbol{\kappa}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\nub}{\boldsymbol{\nu}}
\newcommand{\xib}{\boldsymbol{\xi}}
% omicron (o)
\newcommand{\pib}{\boldsymbol{\pi}}
\newcommand{\varpib}{\boldsymbol{\varpi}}
\newcommand{\rhob}{\boldsymbol{\rho}}
\newcommand{\varrhob}{\boldsymbol{\varrho}}
\newcommand{\sigmab}{\boldsymbol{\sigma}}
\newcommand{\varsigmab}{\boldsymbol{\varsigma}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\upsilonb}{\boldsymbol{\upsilon}}
\newcommand{\phib}{{\boldsymbol{\phi}}}
\newcommand{\varphib}{{\boldsymbol{\varphi}}}
\newcommand{\chib}{\boldsymbol{\chi}}
\newcommand{\psib}{\boldsymbol{\psi}}
\newcommand{\omegab}{\boldsymbol{\omega}}

% Alpha (A)
% Beta (B)
\newcommand{\Gammab}{\mathbf{\Gamma}}
\newcommand{\Deltab}{\mathbf{\Delta}}
% Epsilon (E)
% Zeta (Z)
% Eta (H)
\newcommand{\Thetab}{\mathbf{\Theta}}
% Iota (I)
% Kappa (K)
\newcommand{\Lambdab}{\mathbf{\Lambda}}
% Mu (M)
% Nu (N)
\newcommand{\Xib}{\mathbf{\Xi}}
% Omicron (O)
\newcommand{\Pib}{\mathbf{\Pi}}
% Rho (P)
\newcommand{\Sigmab}{\mathbf{\Sigma}}
% Tau (T)
\newcommand{\Upsilonb}{\boldsymbol{\Upsilon}}
\newcommand{\Phib}{\mathbf{\Phi}}
% Chi (X)
\newcommand{\Psib}{\mathbf{\Psi}}
\newcommand{\Omegab}{\mathbf{\Omega}}


%=========================================================================
% SETS
%=========================================================================
\newcommand{\setA}{\mathcal{A}}
\newcommand{\setB}{\mathcal{B}}
\newcommand{\setC}{\mathcal{C}}
\newcommand{\setD}{\mathcal{D}}
\newcommand{\setE}{\mathcal{E}}
\newcommand{\setF}{\mathcal{F}}
\newcommand{\setG}{\mathcal{G}}
\newcommand{\setH}{\mathcal{H}}
\newcommand{\setI}{\mathcal{I}}
\newcommand{\setJ}{\mathcal{J}}
\newcommand{\setK}{\mathcal{K}}
\newcommand{\setL}{\mathcal{L}}
\newcommand{\setM}{\mathcal{M}}
\newcommand{\setN}{\mathcal{N}}
\newcommand{\setO}{\mathcal{O}}
\newcommand{\setP}{\mathcal{P}}
\newcommand{\setQ}{\mathcal{Q}}
\newcommand{\setR}{\mathcal{R}}
\newcommand{\setS}{\mathcal{S}}
\newcommand{\setT}{\mathcal{T}}
\newcommand{\setU}{\mathcal{U}}
\newcommand{\setV}{\mathcal{V}}
\newcommand{\setW}{\mathcal{W}}
\newcommand{\setX}{\mathcal{X}}
\newcommand{\setY}{\mathcal{Y}}
\newcommand{\setZ}{\mathcal{Z}}


%=========================================================================
% MISCELLANEOUS SYMBOLS
%=========================================================================
\newcommand{\Real}{\mbox{$\mathbb{R}$}}
\newcommand{\Compl}{\mbox{$\mathbb{C}$}}
\newcommand{\VI}{\mathrm{VI}}


%=========================================================================
% OPERATORS
%=========================================================================
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\Diag}{\mathrm{Diag}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\rmF}{\mathrm{F}}
\newcommand{\herm}{\mathrm{H}}
\renewcommand{\Im}{\mathrm{Im}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\rank}{\mathrm{rank}}
\renewcommand{\Re}{\mathrm{Re}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\tran}{\mathrm{T}}
\newcommand{\Var}{\mathrm{Var}}


==> wintech/cost.tex <==
\section{Reproducibility}\label{sec:cost}

%\begin{wrapfigure}{I}{0.45\columnwidth}

%\begin{figure}[t!]
%\centering
%    \includegraphics[width=0.5\columnwidth]{Pic/costs.pdf}
%    \label{fig:costs}
%    \vspace{-4mm}
%    \caption{Cost analysis}
%    \label{fig:cost}
%\end{figure}
%\end{wrapfigure}


\begin{figure}[t!]
\minipage{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{Pic/comp.pdf}
      \vspace{-8mm}
\caption{\small Beamforming gains as a function of the total number of antennas $N$.}
    \label{fig:scalability}
\endminipage
\hfill
\minipage{0.48\columnwidth}
  %\includegraphics[width=\linewidth]{figs/plot_time_snr.pdf}
  \includegraphics[width=\columnwidth]{Pic/costcell.pdf}
    \vspace{-6mm}
  \caption{\small Prototype costs over manufacturing scale.}
  %\vspace{5mm}
  \label{fig:cost}
\endminipage
\end{figure}

To conclude our paper, we provide some final remarks that shall help researchers in the RIS domain build on our results (dataset) and/or reproduce our RIS prototype. 

For starters, we publicly release the dataset\footnote{We will publish the dataset upon the paper acceptance.} we have generated during our empirical characterization in \S\ref{sec:results}, which aggregates a total number of $6.8\cdot 10^6$ power samples. This data can help other researchers study RIS-related problems without the need of building a prototype. 

Next, we report the costs associated for building our prototype. For this purpose, we have used prices publicly available. %xavi that were publicly available on October 10$^{\text{th}}$, 2021.
There are three sources of cost to manufacture each board: ($i$) PCB production (including the patch antenna and the microstrips for the delay lines and the buses); ($ii$) additional electronic components (including RF switches, MCU, resistors, flip-flops, AND gates, etc.); and ($iii$) assembly all components onto the PCB. 

According to {\ttfamily PCBWay}~\cite{PCBWay}, producing 10 PCB boards, as specified in our design, costs \$0.22 per unit cell; but it drops to \$0.11 and \$0.09 when the production scales up by 20x and 100x, respectively. 
%
Concerning additional electronic components, each 10x10 board bears 300 flip-flops, 100 AND gates, 100 RF switches, and 1 MCU. According to {\ttfamily Digikey.de}, the cost boils down to \$1.88 per unit cell when purchasing a batch of 1000 of such boards.
%
The assembly process, according to PCBWay, scales down from \$0.51 to \$0.05 per cell when we scale up the number of boards from 10 to 1000 10x10-RISs. 
%
Fig.~\ref{fig:cost} depicts how these costs (normalized per unit cell) evolve with the manufacturing scale. 
%Note that these prices, summing up to \$184 per unit for the larger batches analyzed here, represent an upper bound of the manufacturing cost as our analysis exclude peer agreements that could lower these prices substantially. 



%\mr{A cost analysis was carried out on 14.10.2021, so all prices are referring to that date. The costs for PCB printing drop down as the quantity increases when purchasing from \cite{PCBWAY}: in our case, for 10 boards the cost was 22.6\$ each, but when the amount is over 200 pieces, the price per board is halved and for 1000 boards it reaches 9.708\$. 

%The cost for the assembly of the components is now taken into account: for 10 boards the cost of the mounting is 51.7\$ per unit, but this cost can be lowered to 6.2\$ for 200 boards and down to 5.2\$ for at least 1000 pieces; after this threshold, the cost is capped and increasing the quantity does not show any decrement. In total, to print and mount the PCB RIS it costs 14.4\$.

%In addition to that, the electronic components must be taken into account. For this calculation, only the main components, meaning only the pieces with high quantity and high prices are considered: they are the MCU, most expensive of them all but there is only per board, flip flops (300 per RIS), AND gates (100 per RIS), and RF-switch (100 per RIS). All the prices are taken from Digikey.de and considering the most convenient batch (usually multiple of 1k or 3k elements), so to realize 1000 RISs, a total of 169\$ per RIS is necessary.

%Hence, a final rough estimated cost for a large scale production of RISs can be 184\$ per unit, however, all the mentioned prices can be negotiated, therefore more favourable prices can be obtained.}


==> wintech/design.tex <==

\section{RIS design}\label{sec:design}

\begin{figure}
\vspace{-2mm}
    \centering
    \includegraphics[width=0.7\linewidth]{Pic/ris_cell_mirror.pdf}
    \vspace{-3mm}
    \caption{\small RIS board and unit cell.}
    \label{fig:unit_cell}
    \label{fig:ris_board}
    %\vspace{2mm}
\end{figure}


The main purpose of our RIS is to perform 3D beamforming passively, i.e., re-focus the energy received from impinging RF signals towards specified directions without active (energy-consuming) RF components. 
%
Fig.~\ref{fig:ris_board} illustrates a \emph{\bf board} consisting of a grid of $N_x \times N_y$ \emph{\bf unit cells} distributed in a 2D array. Unit cells are elements that can reflect RF signals with configurable phase shifts. 
%
%In this way, we can attain 3D beamforming gains passively (without power amplifiers or signal processors). 
%
% the STM32L071V8T6, STM32 offers a Ultra Low-Power segment, the L0 series, ideal for devices powered on battery or for energy harvesting applications \cite{master32}.  Furthermore it permits several communication protocols as SPI, I2C and USART and support Direct Memory Access and Analog to Digital Conversion (ADC).


Phase shifts are configured by a microcontroller unit (MCU), which can be programmed from an external controller.
%
%It is important to select a low-consuming MCU that is friendly to energy harvesting~\cite{ntontin2021autonomous} or other low-power sources.
%
%The MCU can communicate with an external controller with a standard UART interface. 
%Messages are generated from an external access point (AP), in our case a laptop, through a python script.
%
%Since the achievable beamforming gains scale with the number of unit cells~\cite{RISMA}, we cannot afford dedicated connections with the MCU.
Conventional RIS designs are characterized by dedicated $N_x \times N_y$ connections from the MCU to each unit cell. However, MCUs only support a limited number of such connections, which constrains the maximum number of cells and, consequently, the achievable beamforming gains~\cite{RISMA}.
A more scalable approach is to connect each cell with a pair of buses, denoted as \emph{\bf column/row cell selection buses}, that \emph{select} the cell to be configured, and a \emph{\bf phase configuration bus}, which communicates the desired configuration index out of a discrete set. In this way,  we reduce the complexity of the design from $N_x \times N_y$ to $N_x + N_y$ connections per board.
%This approach will maintain the possibility of tuning each antennas individually, at the expense of incrementing a bit the general complexity.

As shown in the right-hand side of Fig.~\ref{fig:ris_board}, each unit cell connects both column/row selection buses with an \emph{\bf AND} gate. Hence, when the MCU sets a high voltage state in row $x$ and column $y$, the MCU activates the configuration bus for unit cell $(x,y)$, whereas all the remaining gates across the board will output a low voltage state ($0$~V).
%In this way, when wishing to configure one individual unit cell, we simply have to select the appropriate pair of row-column cell selection buses. 
%
Each cell also integrates a set of \emph{\bf flip-flop D}, which exploit the high-state exiting the AND gate as a rising edge to update and send out the value stored in memory.
%
We designed our RIS with 3-bit phase shifters, which enable high spatial resolution codebooks. Therefore, each cell uses \emph{three} 1-bit phase configuration buses and \emph{three} flip-flops. 
%the SKY13418-485LF

The latter are connected to \emph{\bf configuration ports} in an \emph{\bf RF switch}. An RF switch is a component that can redirect the RF signal received from an \emph{\bf input port} towards one \emph{\bf output port}, as indicated by the configuration ports. The input port is connected to a \emph{\bf patch antenna}, the ultimate responsible for interacting with the medium, through a \emph{\bf feeding line}.
%This is also shown in Fig.~\ref{fig:unit_cell}.
%
Each output port (except one) uses an open-ended \emph{\bf delay line} with a suitably-designed length to reflect impinging signals with a specific time delay, shifting the signal phase. 

We reserve one output port of the RF switch to connect an \emph{\bf absorber}, an impedance-matching component that absorbs the energy of incoming signals instead of reflecting them back. We call this configuration \emph{absorption state}, and it let us virtually optimize the reflective area of the RIS to meet system constraints. For instance, we can flexibly adapt to different time constraints when optimizing the RIS configuration (which takes longer the larger the number of active cells in the RIS. This is illustrated in Fig.~\ref{fig:adaptive_shapes}.
%
%\mr{optimizing the RIS configuration, either via pre-defined codebooks, or by exploiting instantaneous channel state information, is a complex process that scales with the number of antennas. Hence, there is an incentive to use only the number antennas that you need and not more. To this end, our approach allows to flexibly choose the number of antennas as to obtain the desired trade-off between performance and complexity/overhead.}
%
Alternatively, an energy harvester~\cite{mir2021passivelifi} may be employed instead to re-use the dissipated energy to feed a low-consuming MCU, becoming self-sustainable boards, which we leave for future work.





%The last component of the unit cell is a \emph{patch antenna}, ultimately responsible of interacting with RF signals.  
%The last piece is an RF-switch, the SKY13418-485LF, that is a device that can redirect an RF input to one of its possible outputs; 3 bits, coming as outputs from the flip flops, are used as encoding values and they are passed to the RF-switch to select the desired output port. Each RF-switch output is connected to an open-ended transmission line with its own specific length. Depending on the measure of the transmission line, a delay in time can be added to the signal that will travel throughout the path and subsequently getting a phase shift. So, when a EM waves hit an antenna, the signal travels to the RF-switch, then into a transmission line and it will bounce back to the antenna that will re-radiate the signal with a different phase shift. One of the RF switch output is reserved for a resistor matching the characteristic impedance of line and of the RF-switch to dissipate the incoming signal, that will be not radiated back. The set of AND gate, Flip Flops, RF switch and antenna forms the 'Unit Cell' of the RIS and it is shown in Fig. \ref{unit_cell.}. 
%The element selected to interact with EM waves are \emph{patch antennas}, a particularly cheap antenna with low gain deployed in an array disposition. 
%Each unit cell is connected to an RF switch, which routes the RF input to one possible \emph{delay line}. Each delay line consists of an open-ended transmission line with different length and is responsible to apply a different phase shift to the received signal. 

Our RIS design is modular: as shown in Fig.~\ref{fig:ris_all}, multiple boards can be coordinated through a common bus. The disposition of the unit cells across different boards has been carefully designed to have a separation of $\lambda/2$, where $\lambda$ is the operating wavelength. Such modular boards let us increase/decrease the physical area of our structure without compromising the inter-cell distance, as depicted in Fig.~\ref{fig:adaptive_shapes}.



\begin{figure}[t!]
\vspace{-2mm}
\minipage{0.5\columnwidth}
\centering
  \includegraphics[width=\columnwidth]{Pic/modules.pdf}
    \vspace{-6mm}
  \caption{\small Shape-adaptive RIS.}
  \label{fig:adaptive_shapes}
\endminipage
\hfill
\minipage{0.49\columnwidth}
\centering
  \includegraphics[width=\columnwidth]{Pic/ris_mod_big.pdf}
  \vspace{-7mm}
  \caption{\small Multi-board RIS.}
  \label{fig:ris_all}
\endminipage
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> wintech/lectures.tex <==
\section{lessons learned}

1
Small deviations in the input parameters of models characterizing the characteristic impedance of microstrips yield large empirical errors.


2
Conventional models differ substantially from (full-wave) simulations when estimating the optimal depth of the notch.


3
The operating frequency of patch antennas is very sensitive to deviations in the permittivity $\epsilon_r$ of the substrate material. PCB manufacturers provide a range of $\epsilon_r$ values rather than a precise value, which may lead to large performance errors. Hence, it is worth investing time during the design phase to empirically estimate an accurate $\epsilon_r$ value for the substrate of choice.


4
Precise knowledge of  $v_{\mu \text{strip}}$ is fundamental to design the length of delay lines, and TDR is an essential technique for this purpose. However, for TDR to provide accurate measurements, the samples of microstrips under test should allow the RF signal to travel a distance larger than $2\lambda$. 


5
The ports of the RF switch have a 0.2-mm width, which is smaller than the width of the microstrip lines (0.75~mm). To minimize power loss, it is vital to implement a \emph{smooth} transition, as depicted in Fig.~\ref{fig:RFconnection}~\cite[Table 6]{smooth_line}.


6
The power gain achieved from beamforming scales with the number of cells~\cite{RISMA}. As a consequence, there is a trade-off between the efficiency of an antenna array (negligible mutual coupling when $d_{max} \ge \lambda/2$~\cite{balanis}) and the density of cells in a RIS (higher when $d_{max}\ll\lambda/2$). 
%
Hence, $d_{max} =\lambda/2$ is usually selected. However, mild power loss due to small coupling effects when $d_{max} \lesssim \lambda/2$ may be compensated by the extra cells that this choice permits~\cite{gradoni2021end}.


7
At the beginning of \S\ref{sec:prototype}, we suggested that thin substrates maximize performance. However, we learned that overly thin substrates are considerably harder to manage when assembling electronic components and tend to suffer physical distortions such as warping. 

8
It is conventionally agreed that far-field conditions are ideal for radio characterization. However, doing so for sub-6GHz arrays may be prohibitive. We learned that operating in near-field is good enough as long as we operate beyond the \emph{reactive} near-field threshold, which is less stringent than that of far-field. Prior work usually ignores this aspect~\cite{dai2020reconfigurable, pei2021ris}, which may lead to bad performance.
%Characterizations should be performed in far-field, but for sub-6GHz arrays this is prohibitive because it is in the range of couple of meters. In the literature it is common to carry it out in reactive near-field, but we moved out that zone to get results closer to the theory.  


Considering the size of the codebook and the quasi-static nature of the environment, we learned that collecting 30 samples at a sampling rate of $0.25$~ms$^{-1}$ is a good trade-off between speed and quality of information.  

==> wintech/model.tex <==
\vspace{-1mm}
\section{Beamforming codebook}\label{sec:model}

A RIS board can be modelled as a uniform planar array (UPA) comprised of $N=N_x N_y$ antenna elements~\cite{basar2019wireless, RISMA}. Hence, we define the array response at the RIS for the steering angles $\bar{\theta}$, $\bar{\phi}$ along the azimuth and elevation, respectively, as
\begin{align}
    \a(\bar{\theta},\bar{\phi}) & \triangleq \a_x(\bar{\theta}) \otimes \a_y(\bar{\phi}) \label{eq:UPA}  \\
    & = [1,e^{j2\pi\delta \cos(\bar{\theta})},\ldots,e^{j2\pi\delta(N_x-1) \cos(\bar{\theta})}] \nonumber \\
    & \otimes [1,e^{j2\pi\delta \sin(\bar{\phi})},\ldots,e^{j2\pi\delta(N_y-1) \sin(\bar{\phi})}] \in \Compl^{N\times 1} , \nonumber
\end{align}
where $\delta$ is the ratio between the antenna spacing and the signal wavelength (usually $\delta=0.5$). Assuming line-of-sight signal propagation and a single-antenna transmitter, the channel between the latter and the RIS is given by
\begin{align}
    \g \triangleq \sqrt{\gamma_t}\, \a(\theta_t,\phi_t) \in \Compl^{N\times 1} ,
\end{align}
where we define the average channel power gain as $\gamma_t \triangleq {\beta_0}/{d_t^2}$, with $\beta_0$ the average channel power gain at a reference distance. $d_t$ represents the distance between the transmitter and the RIS, whereas $\theta_t$, $\phi_t$ denote the angles of arrival at the RIS along the azimuth and elevation, respectively. With similar reasoning, the channel between the RIS and the single-antenna receiver is given by
\begin{align}
    \h \triangleq \sqrt{\gamma_r}\, \a(\theta_r,\phi_r) \in \Compl^{N\times 1}.
\end{align}
The matrix containing the RIS configuration is defined as
\begin{align}
    \Phib \triangleq \mathrm{diag}[e^{j\psi_1},\ldots,e^{j\psi_N}] \in \Compl^{N\times N} , \label{eq:Phi_RIS}
\end{align}
with $\psi_n \in \mathcal{Q}, \, \forall n$ and $\mathcal{Q}$ the quantized RIS phase shift set. Note that, to preserve a tractable model in \eqref{eq:Phi_RIS}, we have neglected any phase-dependent reflection coefficient at the RIS. Lastly, the received signal at the receiver is given by
\begin{align}
    y \triangleq \h^\herm \Phib \g \, s + n \in \Compl ,
\end{align}
where $s\in \Compl$ is the transmitted symbol and $n\in \Compl$ is the noise term distributed as $\mathcal{CN}(0,\sigma_n^2)$. 

Let $\v \!\triangleq \!\mathrm{diag}(\Phib^\herm)\!\in\!\Compl^{N\times 1}$ and $\bar{\h} \!\triangleq \!\mathrm{diag}(\h^\herm)\g \!\in\!\Compl^{N\times 1}$, such that the power at the receiver is maximized by letting \cite{ZhangActivePassive}
\begin{align}
    \v = \mathrm{exp}[j \, f_q(\angle \bar{\h})],\label{eq:v_opt}
\end{align}
where $f_q(\cdot)$ projects each element of the vector $\angle\bar{\h}$ in \eqref{eq:v_opt} onto the closest element of set $\mathcal{Q}$ to obtain a feasible solution. 

% OPTION 1:
%It is important to highlight that vector $\bar{\h}$ has the form of a scaling term times the UPA array response in \eqref{eq:UPA} for some steering angles $({\theta},{\phi})$. Hence, in order to design a codebook of RIS beamforming vectors, we artificially create $N_{\mathrm{B}}$ pairs of $\{({\theta_n},{\phi_n})\}_{n=1}^{N_{\mathrm{B}}}$ couples
%within a given search space, where $N_{\mathrm{B}}$ is a design parameter, and generate the corresponding UPA array response vectors $\{\bar{\h}_n\}_{n=1}^{N_{\mathrm{B}}}$.
%Finally, we obtain the RIS configurations $\mathcal{V} := \{\v_n\}_{n=1}^{N_{\mathrm{B}}}$ for each steering angle couple $\{({\theta_n},{\phi_n})\}_{n=1}^{N_{\mathrm{B}}}$ in the codebook by applying the expression in \eqref{eq:v_opt}.
% OPTION 2:
It is important to highlight that vector $\bar{\h}$ has the form of a scaling term times the UPA response vector in \eqref{eq:UPA} for some steering angles $({\theta},{\phi})$. Hence, in order to design a codebook of RIS beamforming vectors, we artificially create $N_{\mathrm{B}}$ pairs of $\{({\theta_n},{\phi_n})\}_{n=1}^{N_{\mathrm{B}}}$ couples and generate the corresponding UPA response vectors $\{\bar{\h}_n\}_{n=1}^{N_{\mathrm{B}}}$. Given the symmetry of the array response around the $x$-axis for the azimuth and around the $y$-axis for the elevation, and in the interest of saving measurement time, we sample a regular grid of points spaced by $3$ degrees in the search space $[-\pi/2,\pi/2]\times[-\frac{\pi}{4},\frac{\pi}{4}]$, such that $N_{\mathrm{B}} = 1891$. Finally, we obtain the RIS configurations $\mathcal{V} := \{\v_n\}_{n=1}^{N_{\mathrm{B}}}$ for each steering angle couple $\{({\theta_n},{\phi_n})\}_{n=1}^{N_{\mathrm{B}}}$ in the codebook by applying the expression in \eqref{eq:v_opt}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> wintech/prototype.tex <==

\section{Prototype Implementation}\label{sec:prototype}
We prototyped our design using a two-layer PCB (Printed Circuit Board). 
%
%PCBs have several advantages, such as low cost, fast production time, and suitability for large-scale implementation.
%
%We selected a 2-layered PCB model.
The substrate material is FR-4, a composite material made of woven fiberglass with an epoxy resin binder that is flame resistant. Its relative electrical permittivity is in the range of  $\epsilon_r = [4.1, 4.8]$, and is coated by two layers of 1-ounce copper (35$~\mu \text{m}$). 
%
In general, thick substrates and high permittivity lead to small bandwidths and low efficiency due to surface waves~\cite{pandey2019practical}. 
%Hence, a thickness between $h=0.003\lambda$ and $h=0.05\lambda$ has to be selected. 
%The operating frequency of our prototype is $f_0=5.3$~GHz ($\lambda=56.56$~mm), which means that the FR-4 thickness should be higher than $0.17$~mm. Hence, we have selected a $h=0.33$~mm thick FR-4 substrate. 
Since the operating frequency of our prototype is $f=5.3$~GHz ($\lambda=56.56$~mm), we chose a substrate thickness of $h=0.53$~mm, that is in the range $0.003 \lambda \leq h \leq 0.05 \lambda$ as suggested in~\cite{pandey2019practical}.



\begin{figure}[b!]
\vspace{2mm}
\minipage{0.49\columnwidth}
\centering
  %\includegraphics[width=\linewidth]{figs/0FAE8C81-1A4E-452D-A180-1404DA39E207.jpeg}
    \includegraphics[width=0.75\columnwidth]{Pic/patch.eps}
    \vspace{-4mm}
\caption{\small Layout of the patch antenna design.}
    \label{fig:patch}
\endminipage
\hfill
\minipage{0.47\columnwidth}
  %\includegraphics[width=\linewidth]{figs/0FAE8C81-1A4E-452D-A180-1404DA39E207.jpeg}
    \includegraphics[width=\columnwidth]{Pic/tdr.pdf}
      \vspace{-8mm}
\caption{\small TDR chart of a 0.95mm-width microstrip.}
    \label{fig:TDR}
\endminipage

\end{figure}



\subsection{Patch Antenna} \label{sec:proto:antenna}
Patch antennas are implemented by cutting out a particular shape from the copper of the board's upper layer. In this way, the remaining metallic shape can radiate at the desired frequency while the back layer operates as ground for the antenna. 
%The patch antenna emits EM waves in front of itself and the backwards radiation is negligible. 
%A patch antenna is not very directive and is linearly polarized following the strip  orientation.
%Our design is shown in Fig.~\ref{fig:patch}.
%
Following the conventional literature on antenna design, we used a rectangular shape, as shown in Fig.~\ref{fig:patch}. In more detail, we used the transmission-line model from \cite{balanis} to calculate its width $W$ and length $L$ as follows:
\begin{align} 
    W &= \frac{\lambda}{2 \sqrt{0.5(\epsilon_r+1)}} = 16.9~\text{mm}, \label{eq:W} \\
    L &= L_{eff} - 2\Delta L = 13.15~\text{mm}, \label{eq:L}
\end{align}
 where $\epsilon_{eff} = \frac{\epsilon_r + 1}{2} + \frac{\epsilon_r - 1}{2} (\frac{1}{\sqrt{1 +12 \frac{h}{w}}})$ is the effective dielectric constant that takes into account the fact that the electric field lines reside in the substrate and partially in the air, $L_{eff} = \frac{c}{2 f \sqrt{\epsilon_{eff}}}$ is the effective length, $c$ is the speed of light, and $\Delta L = 0.412 h \cdot \frac{\epsilon_{eff} + 0.3}{\epsilon_{eff} - 0.258} \cdot \frac{\frac{h}{w} + 0.264}{\frac{h}{w}+0.8}$ is an offset to obtain the antenna physical length from $L_{eff}$ (see \cite{balanis} for details).

As shown in Fig.~\ref{fig:patch}, a microstrip connects each antenna to the RF switch. To this end, we selected an \emph{inset feeding} approach, with a notch at the edge of the antenna. This approach allows us to adapt the antenna to a precise characteristic impedance, which is crucial to maximizing power transfer. Given this notch (see details later), we refined the geometry derived before with the parameters shown in Fig.~\ref{fig:patch} by exhaustive search using a full-wave simulator~\cite{cststudio}, thus setting $W = 15.5~\text{mm}$ and $L = 12.8~\text{mm}$. 
%\begin{align}
%    W &= 15.5~\text{mm}, & L &= 12.8~\text{mm} \nonumber
%\end{align}
%

In the following we describe in detail two crucial parameters, namely ($i$) the width of the microstrip that connects the RF switch (see Fig.~\ref{fig:unit_cell}), and ($ii$) the position of the notch. The former is essential to guarantee impedance-matching, and, since the usual characteristic impedance is 50~$\Omega$, the width of all the microstrips must be selected accordingly. 

\subsubsection{Width of the feeding line}\label{sec:proto:width_lines}

To avoid power loss between the feeding line and the RF switch, their  characteristic impedance should match. 
Therefore, we used the model described in \cite{strip} to estimate a $0.95$-mm line width, which equalizes the $50\Omega$-impedance of the switch. 

%To validate this, we printed a $0.95$mm-width microstrip with an SMA male connector at one end and a $100~\Omega$ resistor at the other end. 
%
%We then used a Vector Network Analyzer (VNA) and applied a Time Domain Reflectometry (TDR) technique to measure the actual characteristic impedance along the sample line. TDR generates a pulse with a short rising time that allows us to calculate the impedance along the line based on the received reflections.
To validate this, we printed a $0.95$mm-width microstrip and applied the Time Domain Reflectometry (TDR) technique using a Vector Network Analyzer (VNA)  to measure the actual characteristic impedance along the line. TDR generates a pulse with a short rising time that allows us to calculate the impedance along the line based on the received reflections.

%By looking at the shape and amplitude of the reflected wave, irregularities (resistor, inductors, shorts, etc.) can be detected. 

As depicted in Fig.~\ref{fig:TDR} (green), this experiment shows that the actual impedance along the line is smaller than the predicted $50~\Omega$. Such a mismatch with the impedance of the switch would incur some power loss at every unit cell and, consequently, poor beamforming gains overall.
%\mr{A charachteristic impedance of $45~\Omega$ would to reflection coefficient $\Gamma=0.0526$, meaning a mismatch loss, the amount of power not available at the output, of 0.01dB.}
%



\begin{figure}[t!]
\minipage{0.49\columnwidth}
\centering
  %\includegraphics[width=\linewidth]{figs/plot_time_snr.pdf}
  \includegraphics[width=0.75\linewidth]{Pic/ff.png}
  \vspace{-4mm}
  \caption{\small Expected radiation pattern of the patch antenna.}
  \label{fig:far_f}
\endminipage
\hfill
\minipage{0.49\columnwidth}
  %\includegraphics[width=\linewidth]{figs/plot_time_snr.pdf}
  \includegraphics[width=\linewidth]{Pic/s11_red.pdf}
    \vspace{-8mm}
  \caption{\small $\boldsymbol{S_{11}}$ parameter of two patch antenna samples.}
  \label{fig:s11}
\endminipage
\end{figure}


Consequently, we opted for a simple empirical approach: we printed out several $135$mm-length microstrips with different widths, and applied the TDR method to each sample.
%
Fig.~\ref{fig:TDR} shows with an orange line the result of the selected sample, with a width equal to 0.75~mm, which provided the best performance.  Ignoring the large oscillation at the beginning of the line, which is due to the soldered SMA connector that we used to connect the line and the VNA, the experiment shows a perfect match with the expected value of $50~\Omega$. 
%Therefore,  we selected this width to implement the feeding line of each unit cell. 



\subsubsection{Notch} 
The second relevant parameter is the depth of the notch, which should minimize the amount of reflected power. This is achieved when the impedance of the antenna matches that of the feeding line. However, the antenna's impedance diminishes as one moves towards its center because the current's intensity is higher at that point. 
Hence, it is important to carefully design the depth of the notch.

Following the analytical method introduced in \cite{balanis}, we first estimated the impedance at the bottom edge of the antenna and centered on the horizontal plane (see red bullet in Fig.~\ref{fig:patch}). At this point, the impedance is purely resistive, i.e., its reactance is zero, and should be equal to  $R_{edge}\approx 341~\Omega$ (we omit the details of the mathematical model, which can be found in \cite{balanis}, to reduce clutter). 
%
Then, the optimal depth of the notch can be computed as:
\begin{align}
    h_{\text{notch}} = \frac{L}{\pi} \cos^{-1}\left( \sqrt{\frac{R}{R_{edge}}}\right) \approx 4.9~\text{mm},
\end{align}
where $R$ is the desired impedance (i.e., $50~\Omega$). 
%This result is practically the same if values for W and L are from Eq. \ref{eq:ant-model} or from our full-wave simulator. 

We attempted to validate this result with the full-wave simulator~\cite{cststudio} and found that a $3.5$-mm depth, cutting across the patch antenna as shown in Fig.~\ref{fig:patch}, maximizes performance ($\sim\!\!30\%$ difference with respect to the model). Fig.~\ref{fig:s11} shows with a blue line the amount of power that is reflected, estimated by the simulator and referred to as S11 parameter in antenna design. The result shows good performance at 5.5~GHz, the operating frequency of choice.
%
%Given our experience with the width of the feed line shown in \S\ref{sec:proto:width_lines}, we decided to use this value instead. 
%
Fig.~\ref{fig:far_f} shows the simulated radiation pattern, with minimal backwards propagation.  Note that the antenna is not very directive and has an expected gain of 1.5dBi, which is common for this type of low-cost antennas.  
%All the remaining parameters of the antenna are summarized in Fig. \ref{fig:patch}. 
%Given all these parameters, Fig.~\ref{fig:far_f} depicts the simulated radiation pattern of each patch antenna. 





To validate the patch design, we printed a sample antenna with the aforementioned parameters. Using our VNA, we measured the empirical $S_{11}$ and plotted the result with a red line in Fig.~\ref{fig:s11}. Perhaps surprisingly, the minimal-$S_{11}$ frequency point is 5.3~GHz instead of the intended 5.5~GHz. After some research, we realized that the offset stems from an error on the nominal permittivity $\epsilon_r=4.3$ used in our model/simulations for the PCB substrate. After some iterations with our simulator, we estimated the real permittivity to be $\epsilon_r=4.66$. In light of this, we changed the operating frequency to $f=5.3$~GHz. 

From Fig.~\ref{fig:s11}, we can also estimate that the bandwidth of our approach, i.e., the range of frequencies where the antenna's $S_{11}$ is $\le-10$~dB, is 118MHz (note the black horizontal line).  We finally note  that, at 5.3~GHz, the $S_{11}$ is $-41$~dB, which corresponds to a Voltage Standing Wave Ration (VSWR) of $1.018$. This means that the amount of power from the feeding line that is reflected back is negligible, which was our goal.
%



\begin{figure}[t!]
\centering
\includegraphics[width=0.6\columnwidth]{Pic/RFconnection.jpeg}
\vspace{-4mm}
\caption{\small RF switch and microstrips.}
\label{fig:RFconnection}
\end{figure}

\setlength\tabcolsep{1.5pt} % default value: 6pt
\begin{table}[t!]
\vspace{-3mm}
\centering
\footnotesize
\begin{tabular}{|r|c|c|c|c|c|c|c|}
\hline
\textbf{Output port}         & 7     & 6      & 5      & 1      & 3      & 2      & 4    \\ \hline
\textbf{$\varphi$ {(}deg{)}} & 51.42 & 102.85 & 154.28 & 205.71 & 257.14 & 308.57 & 360  \\ \hline
\textbf{$l$   {(}mm{)}}       & 1.21  & 2.42   & 3.64   & 4.85   & 6.08   & 7.28   & 8.49 \\ \hline
\end{tabular}
\caption{\small RF switch's output ports, the length of the associated delay lines, and the resulting phase shifts.}
\label{tab:3bitphase}
\vspace{-3mm}
\end{table}



\subsection{Phase shifters} 


At each cell, a specific phase shift $\varphi$ is applied by \emph{routing} the RF signal towards a specific delay line, implemented with a microstrip, that reflects the signal back to the patch antenna. To this end, we use a 3-bit RF switch SKY13418-485LF \cite{SKY}, which has 1 input port (attached to the feeding line), 3 configuration ports (more later), and 8 output ports connected to delay lines of different lengths. Given one configuration (input-output port mapping encoded as 3 bits in the configuration ports), the resulting phase shift follows as:
\begin{equation}
\varphi = \frac{360 \cdot 2l \cdot f}{c \cdot v_f},
\label{phase}
\end{equation}
where $l$ denotes the distance travelled from the patch antenna to the end of the delay line (including the switch and the feeding and delay lines), and $v_f$ is the velocity factor of the microstrip material. 
%
Note that $2l$ accounts for the round-trip between antenna and delay line. 
%

To estimate $v_f$ empirically, we take advantage of the TDR technique used earlier, which also measures the time $d_{\mu \text{strip}}$ it takes for a signal to travel through a microstrip of length $l_{\mu \text{strip}}$. As shown in Fig.~\ref{fig:TDR}, $d_{\mu \text{strip}}= 1.51$~ns for a line of $l_{\mu \text{strip}}=135$~mm, which is sufficiently long to force the signal to travel at least $2\lambda$ and hence enable highly accurate delay estimates. We then calculate $v_f = \frac{v_{\mu \text{strip}}}{c} = 0.298 \approx 0.3$, where $v_{\mu \text{strip}}=\frac{l_{\mu \text{strip}}}{d_{\mu \text{strip}}}$ is the velocity of the signal through the microstrip. 




Given $v_f$ and the selected microstrips width derived in \S\ref{sec:proto:width_lines} ($0.75$~mm), we can calculate the length of the delay lines corresponding to the phase shifts that need to be encoded into each output port, as indicated in Table~\ref{tab:3bitphase}. Note that port 8 has no associated phase shift. Instead, this port connects with a delay line that ends with a $50\Omega$-resistor, which prevents the signal to be reflected back. We refer to this configuration as ``absorption state'', which enables us to build \emph{virtual} RISs of any size and shape. Alternatively, an energy harvester~\cite{mir2021passivelifi} can be used to feed the MCU and effectively make it self-sustainable. The resulting design is shown in  Fig. \ref{fig:RFconnection}. 






\subsection{Microcontroller Unit (MCU)}

As explained in \S\ref{sec:design}, an MCU is in charge of parametrizing the configuration ports of the RF switch in each unit cell.
%
We have selected the STM32L071V8T6 MCU from STMicroelectronics~\cite{mcu}, which is low cost (see \S\ref{sec:cost}), high-speed (configuring 100 cells takes $<35$~ms), and low energy-consuming ($62$~mW in high-performing mode). 
%
We note that we have not optimized the MCU, which we leave for future work. For instance, we only use the MCU's high-performance (high-consuming) mode, although it provides low-consuming modes too. Exploiting these modes could reduce its energy consumption to the order of $\mu$W, which is amenable to energy harvesters~\cite{mir2021passivelifi}. 
%it for maximum performance without exploiting the low-consuming modes available therein.
%However, an optimized MCU (which we leave as future work) could reduce the configuration time substantially and the power consumption to the order of $\mu W$, which is amenable to energy harvesters~\cite{ntontin2021autonomous}. 
%A ST-Link connector is added for enabling the MCU flashing as well an micro USB port for power supply. 
%Push-in terminals are used to create the UART bus and power delivery BUS. The voltage is set to 3.3V by a voltage regulator. The transceiver \cite{RS-485} is essential for UART communication and it has to shorted in case the RIS is the last element of the bus.
%
%To this end, we have programmed the MCU to process AT-formatted control messages sent from an external controller through an UART bus every $1$~ms.


\begin{comment}
We have programmed the MCU to process AT-formatted control messages sent from an external controller through an UART bus every $1$~ms. In addition to standard formatting and error checks, the MCU processes commands with the format shown in Table~\ref{tab:AT}, where `AT' is a prefix; `n' is the board ID; `Y' is the command to execute:
%The MCU is programmed to check for an incoming message every $1$~ms and if the packet is formatted accordingly to the protocol, then it is accepted. UART must be set using the following settings: Baud Rate 115200, Word Length 8 bit, Stop Bits 1 bit, Parity and HW control none. The MCU is set to operate at the fastest speed for the communications, if the communication time is not a constrain, a slower configuration can be chosen in favor of a more power-hungry solution. The packets are structured with AT format:


\begin{itemize}
\item `S': Set phase shift of indicated unit cell;
\item `X': Set phase shift for all unit cells;
\item `R': Reset all unit cells to absorption state;
\item `C': Get average current consumption of the last 10ms;
\end{itemize}
`rr' and `cc' are, respectively, the row and the column with values from `00' to `99'; `O' is the RF switch's output port (1 to 8); and `\textbackslash{}r\textbackslash{}n' is the closing suffix. The time it takes to configure one unit element is on average $35$~ms, but there is room for further optimization.

\begin{table}[h!]
\centering
\vspace{-2mm}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{A} & \textbf{T} & \textbf{n} & \textbf{Y} & \textbf{r} & \textbf{r} & \textbf{c} & \textbf{c} & \textbf{O} & \textbf{\textbackslash{}r} & \textbf{\textbackslash{}n} \\ \hline
\end{tabular}
\caption{\small RIS AT commands} 
\vspace{-10mm}
\label{tab:AT}
\end{table}


\end{comment}


\begin{figure}[t!]
     \centering
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=0.93\textwidth]{Pic/radiation_gain_theta0.png}
         \caption{$\boldsymbol{\theta=0^\circ, \phi=0^\circ}$.}
         \label{fig:ris_0azimuth}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=0.93\linewidth]{Pic/radiation_gain_theta80.png}
         \caption{$\boldsymbol{\theta=80^\circ, \phi=0}$.}
         \label{fig:ris_80azimuth}
     \end{subfigure}
     \vspace{-4mm}
        \caption{\small Expected beamforming pattern of a 10$\boldsymbol{\times}$10 RIS.}
        %\vspace{-2mm}
        \label{fig:ris_azimuth}
\end{figure}


\subsection{RIS board}\label{sec:proto:board}

The spacing between unit cells (antennas) has to be carefully designed to maximize beamforming gains. Roughly speaking, a small spacing increases the probability of mutual coupling, which decreases the efficiency of each antenna because of surface waves propagation. Conversely, a large spacing leads to grating lobes, as we demonstrate in \S\ref{sec:results}. All in all, the inter-cell spacing depends on the maximum steering angle $\theta_{max}$ of the main lobe, which is given by
%\begin{equation}
$
d_{max} = \frac{\lambda}{1+\sin(\theta_{max})} \label{eq:steering}
%\end{equation}
$.
Note that, though $d_{max} =\lambda/2$ maximizes the steering angle range of the array, $\theta_{max}=90^{\circ}$ is not achievable in practice~\citep{AD}. 





 
Prior to developing a prototype, we simulated a $10\times10$ RIS board with a regular $10\times10$ planar antenna array. 
%
%In our first set of simulations, each antenna element is fed with equal power from the open end of a transmission line inducing a phase delay that depends on the selected azimuth and elevation angles.  
In our first set of simulations, each antenna element is fed with equal power from an open-ended transmission line that induces a phase delay that is optimized offline to maximize power towards the selected azimuth and elevation angles.  
%In a full-wave simulator, a 10x10 RIS was recreated utilizing all values previously mentioned and it is shown in Fig. \ref{fullwave_ris}.
%\begin{figure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{Pic/arr.png}
%    \caption{10x10 RIS in a full wave simulator}
%    \label{fullwave_ris}
%\end{figure}
%
Figs.~\ref{fig:ris_0azimuth} and \ref{fig:ris_80azimuth} show the expected radiation pattern of two different configurations that maximize power towards an elevation of $\phi=0^\circ$ and, respectively, an azimuth of $\theta=\{0^\circ, 80^\circ\}$. 

On the one hand, we can observe from Fig.~\ref{fig:ris_0azimuth}  that the array can achieve a narrow beampattern, with a Half Power Beamwidth  (HPBW) equal to $10.1^\circ$, with a gain of $25$~dBi in the intended direction, which halves with a 10-degree offset. No back-radiation is expected. On the other hand, Fig.~\ref{fig:ris_80azimuth} shows that a large steering angle of $\theta=80^\circ$  dissipates half the energy towards the opposite direction and drops the power of the beam to $19.3$~dBi. 

\begin{figure}[t!]
     \centering
     \begin{subfigure}[b]{0.44\linewidth}
         \centering
         \includegraphics[width=0.75\columnwidth]{Pic/rcs0.pdf}
         \vspace{-2mm}
         \caption{$\boldsymbol{0^\circ}$ incidence angle.}
         \label{fig:rcs0}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.44\linewidth}
         \centering
         \includegraphics[width=0.75\linewidth]{Pic/rcs30.pdf}
         \vspace{-2mm}
         \caption{$\boldsymbol{30^\circ}$ incidence angle.}
         \label{fig:rcs30}
     \end{subfigure}
        \vspace{-4mm}
        \caption{\small RCS of a 10$\boldsymbol{\times}$10 RIS illuminated by a plane wave.}
        \label{fig:rcs}
\end{figure}

\begin{figure}[t!]
    \vspace{-4mm}
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\columnwidth]{Pic/10X10_covered.JPEG}
        %\caption{10x10 RIS PCB}
        \caption{RIS board.}
        \label{fig:ris_pcb}        
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{Pic/real_details.jpg}
        %\caption{Testbed in an anechoic chamber with rotating structure.}
        \caption{Testbed.}
        \label{fig:ris_anech}        
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small (a) 10$\boldsymbol{\times}$10 RIS PCB realization, and (b) testbed in an anechoic chamber with rotating structure.}
\end{figure}



Note however that the power radiated by a RIS comes from an external source that \emph{illuminates} the surface. In order to simulate this behavior, we generated a plane wave linearly polarized, and measured the resulting Radar Cross Section (RCS). The RCS estimates how much of the incident power at every point of the surface is scattered back to the receiver. Hence, we expect high RCS values in the direction of the main beam and lower in other directions. This is indeed confirmed in Figs.~\ref{fig:rcs0} and \ref{fig:rcs30} for an incidence angle of $0^\circ$ and $30^\circ$, respectively. In both cases, the RIS is configured to reflect the received signal perpendicularly to the incidence angle of the received signal, i.e., the RIS should maximize power in the same direction of the incidence angle, which is confirmed by both figures with a RCS approximately equal to $12-13$~dBsm in the intended direction.  This highlights the fact that, in real life scenarios, the angle of arrival must be known to the controller to maximize beamforming gains.

 
%\mr{Maybe it is not necessary a subsec for this and can be added before 4.1. For me it is enough to say that this design can be easily readapted for other frequencies in a range as long they are compatible with the operating range of the adopted RF-switch. Once the whole process is known, design again the antenna and the delay line length is not so time-consuming}

We manufactured 10 boards of 10x10 unit cells each. All the phase and selection buses, which connect each unit cell with an MCU, are built with microstrips. Unit cells are deployed in the PCB layout such that the same inter-cell distance can be maintained across co-located boards. The remaining elements described in \S\ref{sec:design} (flip-flops, resistors, etc.), are standard components assembled on the PCB. The final printout is shown in Fig.~\ref{fig:ris_pcb}. 




==> wintech/related.tex <==
%\section{Related Work \ags{target: 0.5 column}}\label{sec:related}


%In this section a brief overview of the RIS prototypes present in the literature are given. In \cite{yezhen2020novel} a 16x16 RIS for 28GHz operating frequency, made of patch antennas connected to a PIN diode which allows only 1-bit resolution phase shift. The maximum scan angle is $\pm$60$^\circ$ and the gain is 21.7dBi. The technology used to control elements is FPGA which permits 2$\mu$s but it increases the overall power consumption with respect to a MCU, in fact the power needed to supply the RIS is 0.8W. \textcolor{blue}{Last sentence not in the paper, from my notes of Sony Lund experience, up to u to keep it.}. The authors of \cite{trichopoulos2021design} show a 16x10 RIS fabricated for 5.8 GHz and the phase shift realized with 1-bit PIN diodes. This prototype does not allow to singularly configure the elements. The control unit, an Arduino MEGA2560, does not support such an amount of elements to be set, therefore the units elements are grouped where each group of 5 elements are configured with the same phase shift. This RIS can achieve a $\pm$60$^\circ$, a bandwidth of 100 MHz and 20dB SNR in some scenarios. In \cite{tan2018enabling}, a RIS prototype consisting of 14x16 reflectors is presented with center frequency at 60 GHz. The unit elements are place more than one wavelength away to reduce the mutual coupling at the expense a tight maximum scanning angle. To set the phase shifts, a switch is involved: when it is open, the patch is isolated from the ground plane and it is reflecting, when it is closed, the antenna is shorted to the ground and it has minimum reflection. However the authors of this paper do not show any characterization of their RIS. Several MIMO prototypes are described in \cite{clerckx2022foundations} for wireless power transfer purposes and a RIS designed is shown to enhance the efficiency and extend the operational range. The adapted RIS contains 16x16 elements working at 5.8GHz equipped with a PIN diode for 1-bit control. The unit cells are controlled by a FPGA which sets the phase shift in shift registers. Unfortunately no information is given about the performance of this RIS. Of particular interest is the prototype presented in \cite{dai2020reconfigurable} because a 2-bit phase quantization is obtained using 5 PIN diodes. The RIS consists of 3 layers: the ground, the slotted plane, and the patch reflector. The length of the resonant slots is changed by activating the diodes and therefore applying different phase delay. This prototype has 16x16 elements and it is command by an FPGA. The achievable gain at 2.4 GHz is 21dBi and the main beam can be scanned up to $\pm$60$^\circ$. Also it is stated that if the radiated power is 18dB, the RIS power consumption is 153 W. In \cite{arun2020rfocus}, 40 reflectors are mounted on the boards, they are $\lambda/4$ tall, $\lambda/10$ wide and separated $\lambda/10$ on x-axis and on the y-axis just enough to connected by an RF-switch. When the switch is turned on, they reflectors form an half dipole antenna resonating at 2.4GHz. The authors put together 80 boards but they did not disclose the key parameters. A very peculiar layout was created in \cite{pei2021ris}, where a 3-layered RIS with 1100 elements is revealed that operates at 5.8GHz. An unit element consists of 4 reflectors where a PIN diode link the first two reflectors and another diode the second two. By changing the biasing voltage the authors claim the continuous phase shifts in a span of 180$^\circ$ is possible, but they limit their choice to only two value to apply a 1-bit phase shift. Given they high quantity of elements in the board, all the units on the same column are grouped together and set by an FPGA with the same phase shift. It is noteworthy the 500m field trial where a film was streamed smoothly, the RIS allowed power gain of 14 dB. The total power consumption for this RIS is 0.9W. A very similar approach is illustrated in \cite{scattermimo} to allow singular configuration of the elements reducing the number of utilized pins at controller side. This RIS is made of 4x4 patch antennas operating at 5 GHz and controlled with 2-bit phase shifter made with the transmission line method. They claim that this prototype can double the average throughput gain and increase the coverage from 30m to 45m in indoor environment. The total power consumption for it 12mW.

==> wintech/results.tex <==



\begin{figure}[t!]
    \centering
    \includegraphics[width=0.7\columnwidth]{Pic/testbed10.pdf}
    \vspace{-4mm}
    \caption{\small Map of the testbed.}
    \label{fig:testbed}
\end{figure}


\vspace{-3mm}
\section{Empirical Characterization}\label{sec:results}


We characterized one of our 10x10 RIS boards in an 8m$\times$5m anechoic chamber. Figs.~\ref{fig:ris_anech} and \ref{fig:testbed} illustrate our testbed. 
%
We mounted the board on a turntable controlled remotely from a master PC, which is also used to configure the beamforming parameters of the RIS. 
%
We use two software-defined radio devices attached to horn antennas with gain $G=13.5$~dBi to generate (``TX'') and receive (``RX'') a continuous stream of OFDM QPSK-modulated symbols with 5~MHz of bandwidth and numerology that meets 3GPP LTE requirements. 
%
%The transmission power of TX is set to 8~dBm, and we sample the reference signal received power (RSRP) at RX. 
The transmission power of TX is -30~dBm per subcarrier, and we sample the reference signal received power (RSRP) at RX. 

The distances RIS-TX and RIS-RX are $d_{\text{RIS}-\text{TX}}\!=\!1.1$~m and $d_{\text{RIS}-\text{RX}}\!=\! 6.3$~m, respectively. Considering the size of the RIS and its operating frequency, it is hard to guarantee that $d_{\text{RIS}-\text{TX}}$ is larger than the far-field threshold, which is $2\frac{D^2}{\lambda}\!=\!6.5$~m~\cite{balanis}, where $D\!=\!0.43$~m is the diagonal of the array. Nevertheless, our choice of $d_{\text{RIS}-\text{TX}}$ is larger than the \emph{reactive} near-field threshold, which is $0.62\sqrt{\frac{D^3}{\lambda}}\!=\!0.73$~m~\cite{balanis}, and sufficient for our purposes.
%
As shown in Fig.~\ref{fig:testbed}, the rotation of the table determines the azimuth angle $\theta_r$, and the location of TX determines $\theta_t$. Conversely, the elevation angles of RIS-TX and RIS-RX are fixed to $\phi_t \!=\! 33^{\circ}$ and $\phi_r \!=\! -3^\circ$, respectively. 




\vspace{-1mm}
\subsection{Codebook characterization}

\begin{figure}[t!]
     \centering
     \includegraphics[width=\columnwidth]{Pic/AoA0_shift.pdf}
    \vspace{-14mm}
     \caption{Examples of beampatterns for $\boldsymbol{\theta_t=0^\circ}$.}
     \label{fig:pattern:1}
    %\vspace{-2mm}
\end{figure} 

We begin our experimental campaign by characterizing the codebook generated in \S\ref{sec:model}. 
%Our codebook consists of a total of $N_B = 1891$ configurations, which should cover the search space specified in \S\ref{sec:model} with a granularity of $3^\circ$ (i.e., $$
To this end, we test out all the configurations $\mathcal{V} = \{\v_n\}_{n=1}^{N_{\mathrm{B}}=1891}$ for a wide range of $\theta_r=[-90^{\circ}, 90^{\circ}]$ and for $\theta_t=\{20^{\circ}, 90^{\circ}\}$. 







For our empirical results, the first observation is that the direction $(\theta_n, \phi_n)$ of the main lobe points towards $(\theta_r- \theta_t, \phi_r- \phi_t)$, as intended, for all configurations $\v_n\in\mathcal{V}$. These results, hence, validate our prototype for practically all configurations in $\mathcal{V}$. 
Figs.~\ref{fig:pattern:1} and \ref{fig:pattern:2} depict some representative configurations $\v_n\in\mathcal{V}$ for both $\theta_t$ settings, respectively. These figures show that the main beam points towards the intended directions.
%
%When $\theta_t=0^{\circ}$, we can observe that the RIS maximizes power in the direction of $\theta_r=\theta$, as intended, because TX is perpendicular to the RIS in this case.
%
%The configuration that maximizes power is $\phi=-30^\circ$ (selected for all the plots in Figs.~\ref{fig:pattern:1} and \ref{fig:pattern:2}). This is expected because $\phi=-30^\circ$ compensate the value of $\phi_t=33^{\circ}$, which is fixed in our setup. 
%
%Similarly, we can observe that the azimuth direction $\theta_r$ of the main lobe points towards $\theta-\theta_t$, which validates our prototype for all configurations in $\mathcal{V}$. 
%Perhaps more surprising is the fact that, when $\theta_t=0^{\circ}$ (Fig.~\ref{fig:pattern:1}) the maximum gain is achieved for $\theta=-12^{\circ}$ (and not $\theta=0^{\circ}$), with an observed received power of 24~dBm; and when  $\theta_t=20^{\circ}$ (Fig.~\ref{fig:pattern:1}), that is achieved for  $\theta=-12^{\circ}$ (and not $\theta=0^{\circ}$), observing \ags{xx}~dBm.  This may be explained because \tbd{...}. 
% 
We note, however, that the gain of the main lobe is penalized when we use large steering angles (see, e.g., $\theta=60^{\circ}$ in both figures), which is expected~\cite{AD}. 
%In the most extreme case, Fig.~\ref{fig:pattern:2}'s $(\theta=60^\circ, \phi=-30^\circ)$, the steering azimuth angle is so pronounced ($\theta_t+\theta = 80^\circ$) that substantial power is reflected towards other directions, which is in line with our simulations in \S\ref{sec:design} (see Fig.~\ref{fig:ris_80azimuth}).
%
Overall, the power received in the intended direction ranges between $-74$~dBm (for large steering angles) and $-64$~dBm (for smaller angles), which give us remarkable beamforming gains between $\sim\!17$~dB and $\sim\!27$~dB over the noise floor. 

Using the radar range equation in \cite{balanis}, the peak RCS can be calculated as
$
64\pi^3 \frac{P_{RX}}{P_{TX}} \cdot (\frac{d_{\text{RIS}-\text{TX}} \cdot d_{\text{RIS}-\text{RX}}}{\lambda \cdot G})^2
= 11.2$~dBm$^2$. Moreover, the HPBW is in average around $10^\circ$ for all beampatterns. Both results are in line with our simulations in \S\ref{sec:proto:board}. 
%}.

%(i used -64dbm as Prx, but then we say in sec 5.2 that Prx is -66.5 dbm. Using the second value rcs is -11.2dbsm) 



\begin{figure}[t!]
     \centering 
     \includegraphics[width=\columnwidth]{Pic/AoA20_shift.pdf}
    \vspace{-14mm}
     \caption{Examples of beampatterns for $\boldsymbol{\theta_t=20^\circ}$.}
     \label{fig:pattern:2}
    %\vspace{-2mm}
\end{figure}

%\mr{
%At the first stage, a codebook is generated as discussed in Sec. \ref{sec:model}: it consists of 1891 configurations, where each of them steers the main beam of the RIS to a precise position expressed as ($\theta,\phi$), with $\theta$ indicating the azimuth and $\phi$ the elevation. In detail, the main beam is scanned for $\theta$ from $-90^{\circ}$ to $90^{\circ}$ and for $\phi$ from $-45^{\circ}$ to $45^{\circ}$, both with a step of $3^{\circ}$. This codebook was tested for each location of the table to compute a radiation pattern for every configuration. In particular, for each configuration 30 power samples with a rate of 4ms are collected. The procedure is repeated for $\theta_t=0^{\circ}$ and $\theta_t=20^{\circ}$.


%The results for these experiments are shown in Fig. \ref{fig:pattern:1}-\ref{fig:pattern:2} and for both the received power is maximized for the configuration steering the main beam to ($\theta=-12^{\circ},\phi=-30^{\circ}$) reaching 24dBm. The elevation angle of the best configuration was expected because it has to compensate for the elevation of the TX-RIS and RIS-RX links, but for the azimuth there is an offset \mr{dont know how to justify/explain this yet}. The sidelobes seem to have significant values, but they remain constant when main beam is steered to $\pm60$ and beyond without showing signs of multiple main lobes. This trend is confirmed for both AoA. However, it is noteworthy to highlight that changing the AoA is shifting the location of the main beam in accordance with $\theta_t$.
%}

\vspace{-1mm}
\subsection{Scalability analysis}



\begin{figure}[t!]
\vspace{-4mm}
     \centering
     \begin{subfigure}[b]{0.15\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{Pic/2x2.pdf}
         \caption{2x2}
         \label{fig:activation:1}
     \end{subfigure}
     \begin{subfigure}[b]{0.15\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{Pic/4x4.pdf}
         \caption{4x4}
         \label{fig:activation:2}
     \end{subfigure}
     \begin{subfigure}[b]{0.15\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{Pic/8x8.pdf}
         \caption{8x8}
         \label{fig:activation:3}
     \end{subfigure}
     \begin{subfigure}[b]{0.15\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{Pic/10x10.pdf}
         \caption{10x10}
         \label{fig:activation:4}
     \end{subfigure}     
     \begin{subfigure}[b]{0.15\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{Pic/off2.pdf}
         \caption{off2}
         \label{fig:activation:5}
     \end{subfigure}  
     \begin{subfigure}[b]{0.15\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{Pic/off3.pdf}
         \caption{off3}
         \label{fig:activation:6}
     \end{subfigure}     
    \vspace{-4mm}
        \caption{\small Different unit cell activation patterns in a 10x10 RIS board. Colored squares represent deactivated (in black) and activated (in white) cells.}
        \label{fig:activation}
\end{figure}



To assess scalability, we analyze the beamforming gain of our RIS for a variable number of unit cells. To this goal, we take advantage of the  absorption state available in our design  for each cell, and produce virtual RISs with different sizes by setting the activation patterns shown in Figs.~\ref{fig:activation:1} to \ref{fig:activation:4}. For every virtual RIS, we re-optimized its codebook $\mathcal{V}_{N}$ to account for its effective size and inter-cell spacing. 

To ease the analysis, we now fix $\theta_r=\theta_t=0^\circ$ and measure the power received for every configuration $\v\in\mathcal{V}_N$. The results are shown in Fig.~\ref{fig:vRISs}, which represent the measured power with a color range for every combination of $\theta$ (x-axis) and $\phi$ (y-axis) from $\mathcal{V}_N$, and for $N=\{4, 8, 64, 100\}$. 
%
From these plots, we can observe how the main beam becomes sharper and carries more power as we increase $N$. With $N=4$ (top left plot), no configuration produces a distinguishable beam, which renders a 2x2 RIS ineffective. For the rest, we note a growing amount of power in the intended direction, respectively, equal to $-81.8$~dBm ($N=16$), $-71.5$~dBm ($N=64$), and $-66.5$~dBm (all cells are activated). This behavior is expected: Fig.~\ref{fig:scalability} depicts in red the power observed at RX with the optimal configuration $\v$ as a function of $N$, and compares that with the mathematical model in \cite{9206044} (see eq.~(5) therein) represented in blue. Both results are remarkably close to each other, which validates the ability of our approach to effectively create virtual surfaces with different shapes.


\begin{figure}[t!]
  \centering
    \includegraphics[width=\columnwidth]{Pic/rp_2x2_shift.pdf}
    \vspace{-8mm}
    \caption{\small Received power over the respective optimal codebook $\boldsymbol{\mathcal{V}_N}$ for virtual RISs with different sizes (activation patterns of Figs.~\ref{fig:activation:1}-d, respectively). $\boldsymbol{\theta_r=\theta_t=0^\circ}$.}
  \label{fig:vRISs}
\end{figure}

%\mr{
%As second stage, the absorption mode capability of RIS is tested by trying to turn off elements following predefined patterns. In particular, virtual subarrays are created to verify how the number of active elements affects the amount of received power and the sharpness of the main beam. These patterns are illustrated in Fig. \ref{fig:activation:1}-d. Afterwards, the absorption mode is enabled for some consecutive rows and columns, in such a way the inter-element distance is greater than $\lambda$ and the grating lobes effect is experienced. In Fig. \ref{fig:activation:5}-f it can be seen that one row (column) is followed by 2 or 3 rows (columns) with turned off elements, imposing the inter-element distance, $d$, to $1.5\cdot\lambda$ and $2\cdot\lambda$.

%The results after creating virtual squared subarrays are shown in Fig. \ref{fig:heats}. It is clear that in the 2x2 case, the amount of antennas is not enough to generate beamforming, but from the 4x4 scenario a weak beamforming is starting to occur. For the two remaining plots, instead, it is evident that the beamforming is operating as expected. Thanks to these figure, it is confirmed that the received power increases, as expected, with the number of the active elements. Furthermore, the area with highest received power gets narrower with number of active elements, since the mainbeam gets sharper. 
%}

\subsection{Other activation patterns}

\begin{figure}[b!]
     \centering
     \begin{subfigure}[b]{0.495\columnwidth}
         \centering
         \includegraphics[width=1.05\columnwidth]{Pic/OffSpace2_shift.eps}
         \vspace{-7mm}
         \caption{$\boldsymbol{d_{max}=\lambda}$.}
         \label{fig:off2}
     \end{subfigure}  
     \begin{subfigure}[b]{0.495\columnwidth}
         \centering
         \includegraphics[width=1.05\columnwidth]{Pic/OffSpace3_shift.eps}
         \vspace{-7mm}
         \caption{$\boldsymbol{d_{max}=1.5\lambda}$.}
         \label{fig:off3}
     \end{subfigure}     
    \vspace{-6mm}
        \caption{\small Received power over the respective optimal codebook $\boldsymbol{\mathcal{V}_{d_{max}}}$ for virtual RISs generating grating lobes (activation patterns of Figs.~\ref{fig:activation:5}-f, respectively). Red dots indicate the expected location of the lobes. $\boldsymbol{\theta_r=\theta_t=0^\circ}$.}
        \label{fig:grating}
\end{figure}

To conclude our characterization, we study the performance of our RIS prototype when the inter-cell distance differs from $d_{max}=\lambda/2$ (shown in Fig.~\ref{fig:vRISs} for $N=100$).   Like before, we calculated new optimized codebooks $\mathcal{V}_{d_{max}}$ for $d_{max}=\{\lambda, 1.5\lambda\}$, and plot in Fig.~\ref{fig:grating} the power received at RX for each configuration $\v\in\mathcal{V}_{d_{max}}$. We do this for both activation patterns depicted in Fig.~\ref{fig:activation:5} (``off2'') and \ref{fig:activation:6} (``off3''), for $d_{max}=\lambda$ and $d_{max}=1.5\lambda$, respectively. 

By changing $d_{max}$, we also change the density of active cells per board, $N=25$ for $d_{max}=\lambda$ (Fig.~\ref{fig:off2}) and $N=16$ for  $d_{max}=1.5\lambda$ (Fig.~\ref{fig:off3}). As shown earlier, this has a cost in terms of beamforming gains that is evidenced also in Fig.~\ref{fig:grating}: the maximum power is $-80.4$~dBm and $-84.2$~dBm for the two cases, respectively. 
%
Both plots reveal the presence of grating lobes, which are symmetrical beams that are denser for larger  $d_{max}$ values. 
%
These effects are well understood in the literature of antenna design and their distance can be estimated using our model in \S\ref{sec:model}. The figure depicts with red circles the expected location of these lobes, which match our measurements remarkably well. This further validates our design to effectively modify the shape of the RIS to the requirements of any given use case. 
%These reflections are well understood in the literature of antenna design and their distance can be estimated with $d_m:=\arcsin(\frac{m  \cdot \lambda}{d_{max}})$ with $m\in \{0, 1, 2, \dots\}$~\cite{AD}. In our setup, this model yields $d_{grating}=\pm42^{\circ}$ for Fig.~\ref{fig:off2} and $d_{grating}=\pm30^{\circ}$ for Fig.\ref{fig:off3}, which agrees with our results in Fig.~\ref{fig:grating}, and shows how our design is able to effectively modify the shape of the RIS to adapt to the requirements of any given use case. \ags{theory does not match that well!}

%\mr{
%Fig. \ref{fig:off2}-b depict respectively the results for turning off two and three consecutive rows/columns. It is possible to see for both that multiple high power regions are present with a periodic pattern; the former shows higher power, because more elements were left active. The horizontal distance between peaks can be estimated mathematically with $\arcsin(m \cdot \frac{\lambda}{d})$ with $m\in \mathbb{N}_0$. Since the argument must be in the range [-1,1], the formula yields a distance of $42^{\circ}$ for Fig. \ref{fig:off2} and of $30^{\circ}$ for Fig. \ref{fig:off3}, which seems to be roughly respected. \mr{compare with placidos plot?}  
%}



